BoIR: Box-Supervised Instance Representation for Multi-Person Pose Estimation

Single-stage multi-person human pose estimation (MPPE) methods have shown great performance improvements, but existing methods fail to disentangle features by individual instances under crowded scenes. In this paper, we propose a bounding box-level instance representation learning called BoIR, which simultaneously solves instance detection, instance disentanglement, and instance-keypoint association problems. Our new instance embedding loss provides a learning signal on the entire area of the image with bounding box annotations, achieving globally consistent and disentangled instance representation. Our method exploits multi-task learning of bottom-up keypoint estimation, bounding box regression, and contrastive instance embedding learning, without additional computational cost during inference. BoIR is effective for crowded scenes, outperforming state-of-the-art on COCO val (0.8 AP), COCO test-dev (0.5 AP), CrowdPose (4.9 AP), and OCHuman (3.5 AP). Code will be available at https://github.com/uyoung-jeong/BoIR

==> figures/1_pipeline_export.tex <==
\begin{tabular}{c@{\hspace{0.3em}}c}
\raisebox{-0.5\height}{
\begin{tikzpicture}[thick,scale=0.7, every node/.style={transform shape}]
\tikzstyle{connection}=[ultra thick, every node/.style={sloped,allow upside down, minimum size=1em},draw=\edgecolor,opacity=0.7]
% f
\node[canvas is xy plane at z=0] (f) at (0,0,0) {$f$};

% neck
\node[shift={(0,1.0,0)},fill=blue!40,minimum width=1,minimum height=1.4em,font=\small] at (f.north) (neck) {ASPP};

% center head
\node[shift={(0,1.0,0)},fill=blue!40,minimum width=1,minimum height=1.4em,font=\small] at (neck.north) (center_head) {center};

% buk head
\node[shift={(1.5,1.0,0)},fill=cyan!40,minimum width=1,minimum height=1.4em,font=\small] at (neck.north) (buk_head) {buk};

% bbox head
\node[shift={(2.5,1.0,0)},fill=cyan!40,minimum width=1,minimum height=1.4em,font=\small] at (neck.north) (bbox_head) {bbox};

% emb head
\node[shift={(3.5,1.0,0)},fill=cyan!40,minimum width=1,minimum height=1.4em,font=\small] at (neck.north) (emb_head) {emb};

% center
\node[shift={(0,0.5,0)},minimum width=1,minimum height=1.4em,font=\small] at (center_head.north) (center) {$c$};

% buk
\node[shift={(0,0.5,0)},minimum width=1,minimum height=1.4em,font=\small] at (buk_head.north) (buk) {$k^{bu}$};

% bbox
\node[shift={(0,0.5,0)},minimum width=1,minimum height=1.4em,font=\small] at (bbox_head.north) (bbox) {$b$};

% emb
\node[shift={(0,0.5,0)},minimum width=1,minimum height=1.4em,font=\small] at (emb_head.north) (emb) {$e$};

% parameter sampling
\node[shift={(-1.0,0,0)},fill=orange!40,minimum width=1,minimum height=1.4em,font=\small] at (center.west) (sample) {sample};

% f^p
\node[shift={(-0.71,0,0)},minimum width=1,minimum height=1.4em,font=\small] at (sample.west) (fp) {$f^p$};

% kpt head
\node[shift={(-0.805,0,0)},fill=blue!40,minimum width=1,minimum height=1.4em,font=\small] at (fp.west) (kpt_head) {kpt};

% kpt
\node[shift={(0,0.5,0)},minimum width=1,minimum height=1.4em,font=\small] at (kpt_head.north) (kpt) {$k$};

% kpt loss
\node[shift={(0,1.0,0)},minimum width=1,minimum height=1.4em,font=\small, text=orange] at (kpt.north) (kpt_loss) {$\mathcal{L}_{kpt}$};

% center loss
\node[shift={(0,1.0,0)},minimum width=1,minimum height=1.4em,font=\small, text=orange] at (center.north) (center_loss) {$\mathcal{L}_{center}$};

% buk loss
\node[shift={(0,1.0,0)},minimum width=1,minimum height=1.4em,font=\small, text=orange] at (buk.north) (buk_loss) {$\mathcal{L}_{buk}$};

% bbox loss
\node[shift={(0,1.0,0)},minimum width=1,minimum height=1.4em,font=\small, text=orange] at (bbox.north) (bbox_loss) {$\mathcal{L}_{bbox}$};

% emb loss
\node[shift={(0,1.0,0)},minimum width=1,minimum height=1.4em,font=\small, text=orange] at (emb.north) (emb_loss) {$\mathcal{L}_{emb}$};

% dashed box
\begin{pgfonlayer}{background}
\node[draw=gray,dashed,fill=gray!1,thick, inner sep=5pt,fit=(buk_head) (bbox_head) (emb_head) (buk) (bbox) (emb) (buk_loss) (bbox_loss) (emb_loss)] (trim) {};
\node[shift={(0,0.25,0)},minimum width=1,font=\scriptsize] at (trim.north) (dashed_box_caption) {Removed in inference phase};

\end{pgfonlayer}
% connections
\draw [-Stealth]  (f.north)    -- (neck.south);
\draw [-Stealth]  (neck.north)    -- (center_head.south);
\draw [-Stealth]  (neck.north) -- ++(0,0.5,0)  -- ++(1.5,0,0)  -- (buk_head.south);
\draw [-Stealth]  (neck.north) -- ++(0,0.5,0) -- ++(2.5,0,0)  -- (bbox_head.south);
\draw [-Stealth]  (neck.north) -- ++(0,0.5,0) -- ++(3.5,0,0)  -- (emb_head.south);

\draw [-Stealth]  (center_head.north)    -- (center.south);
\draw [-Stealth]  (buk_head.north)    -- (buk.south);
\draw [-Stealth]  (bbox_head.north)    -- (bbox.south);
\draw [-Stealth]  (emb_head.north)    -- (emb.south);

\draw [-Stealth]  (f.north) -- ++(0,0.5,0) -- ++(-1.2,0,0)  -- (sample.south);
\draw [-Stealth]  (f.north) -- ++(0,0.5,0) -- ++(-3.6,0,0)  -- (kpt_head.south);
\draw [-Stealth]  (center.west)    -- (sample.east);
\draw [-Stealth]  (sample.west)    -- (fp.east);
\draw [-Stealth]  (fp.west)    -- (kpt_head.east);
%\draw [-Stealth]  (center.west) -- (kpt_head.east);
\draw [-Stealth]  (kpt_head.north)    -- (kpt.south);

\draw [-Stealth, fill=orange,draw=orange]  (kpt_loss.south)    -- (kpt.north);
\draw [-Stealth, fill=orange,draw=orange]  (center_loss.south)    -- (center.north);
\draw [-Stealth, fill=orange,draw=orange]  (buk_loss.south)    -- (buk.north);
\draw [-Stealth, fill=orange,draw=orange]  (bbox_loss.south)    -- (bbox.north);
\draw [-Stealth, fill=orange,draw=orange]  (emb_loss.south)    -- (emb.north);
\end{tikzpicture}} &
\raisebox{-0.5\height}{
\input{figures/5_ikh_comp}
}
\end{tabular}

==> figures/4_ikh_pipeline.tex <==
\begin{tikzpicture}[thick,scale=0.8, every node/.style={transform shape}]
\tikzstyle{connection}=[ultra thick,every node/.style={sloped,allow upside down, minimum size=1em},draw=\edgecolor,opacity=0.7]
% f
\node[canvas is xy plane at z=0] (f) at (0,0,0) {$f$};

% center
\node[shift={(0,-0.5,0)},minimum width=1,minimum height=1.4em,font=\small] at (f.south) (center) {$c$};

% parameter sampling
\node[shift={(1.0,0,0)},fill=orange!40,minimum width=1,minimum height=1.4em,font=\small] at (center.east) (sample) {sample};

% f^p
\node[shift={(0.71,0,0)},minimum width=1,minimum height=1.4em,font=\small] at (sample.east) (fp) {$f^p$};

% kpt head
\node[shift={(2.29,0,0)},fill=blue!40,minimum width=1,minimum height=1.4em,font=\small] at (f.east) (kpt_head) {kpt};

% kpt
\node[shift={(0.5,0,0)},minimum width=1,minimum height=1.4em,font=\small] at (kpt_head.east) (kpt) {$k$};

% connections
\draw [-Stealth]  (f.east) -- (kpt_head.west);
\draw [-Stealth]  (f.east) -- (sample.west);
\draw [-Stealth]  (center.east) -- (sample.west);
\draw [-Stealth]  (sample.east)    -- (fp.west);
\draw [-Stealth]  (fp.north)    -- (kpt_head.south);
\draw [-Stealth]  (kpt_head)    -- (kpt.west);
\end{tikzpicture}

==> rebuttal/bbox_mask_loss_vis.tex <==
\begin{figure}
\centering
\begin{tabular}{cccc}
CID & Sim. & BoIR & Sim. \\
\includegraphics[width=0.18\linewidth]{rebuttal/images/cid_000000404678_0.png} & \includegraphics[width=0.18\linewidth]{rebuttal/images/cid_000000404678_1.png} & \includegraphics[width=0.18\linewidth]{rebuttal/images/boir_000000404678_0.png} & \includegraphics[width=0.18\linewidth]{rebuttal/images/boir_000000404678_1.png} \\ 
\end{tabular}
\caption{Visualization of feature similarities from COCO val. Activated region is marked with red circle. Leftmost: CID's keypoint prediction. Second: CID's feature similarity from the instance center. Third: BoIR's keypoint prediction. Rightmost: BoIR's feature similarity from the instance centers.
\vspace*{-5mm}}
\label{fig:bml_overlap_vis}
\end{figure}

%\begin{figure}
%\begin{center}
%\begin{tabular}{cccc}
% & Keypoint & Inst. 1 Sim. & Inst. 2 Sim. \\
%\rotatebox[origin=c]{90}{CID} & \raisebox{-.5\height}{\includegraphics[width=0.25\linewidth]{rebuttal/images/cid_000000404678_0.png}} & %\raisebox{-.5\height}{\includegraphics[width=0.25\linewidth]{rebuttal/images/cid_feat_sim_2_0.218_000000404678_1.png}} & \\
%\rotatebox[origin=c]{90}{BoIR} & \raisebox{-.5\height}{\includegraphics[width=0.25\linewidth]{rebuttal/images/boir_000000404678_0.png}} & %\raisebox{-.5\height}{\includegraphics[width=0.25\linewidth]{rebuttal/images/boir_feat_sim_3_0.152_000000404678_1.png}} & \raisebox{-.5\height}%{\includegraphics[width=0.25\linewidth]{rebuttal/images/boir_feat_sim_6_0.067_000000404678_2.png}} \\ 
%\end{tabular}
%\end{center}
%\caption{Visualization of feature similarities on overlapping instances from COCO val set. First column: keypoint detection results. Second %column: backbone feature similarity heatmap for detected instance 1(a baby) center. Third column: backbone feature similarity heatmap for %detected instance 2(a person holding the baby) center.}
%\label{fig:bml_overlap_vis}
%\end{figure}

==> rebuttal/fig_merged.tex <==
%\begin{figure*}
%\begin{figure*}
\begin{strip}
%\begin{figure}[!ht]
\centering
\small{
\begin{tabular}{c@{}c@{}c@{}c@{}c@{}c@{}c@{}c}
\includegraphics[width=0.122\linewidth]{rebuttal/pdfs/bml_framework.pdf} &
%\includegraphics[width=0.132\linewidth]{rebuttal/images/graphical_bml.png} &
\includegraphics[width=0.15\linewidth]{rebuttal/pdfs/pipeline.pdf}
 & %%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.28\linewidth]{rebuttal/pdfs/comp.pdf} &

\includegraphics[width=0.089\linewidth]{rebuttal/images/BikerWithBoxR.png} & 
\includegraphics[width=0.089\linewidth]{rebuttal/images/CIDAR.png} & 
\includegraphics[width=0.089\linewidth]{rebuttal/images/CIDBR.png} &  
\includegraphics[width=0.089\linewidth]{rebuttal/images/BoIRAR.png} &
\includegraphics[width=0.089\linewidth]{rebuttal/images/BoIRBR.png}\\
%\includegraphics[width=0.10\linewidth]{rebuttal/images/BoIRB.png} &
%\includegraphics[width=0.21\linewidth]{rebuttal/pdfs/pipeline.pdf}
% & %%%%%%%%%%%%%%%%%%%%
%\includegraphics[width=0.16\linewidth]{rebuttal/pdfs/comp.pdf}
%&
%\includegraphics[width=0.08\linewidth]{rebuttal/images/cid_000000314251_0.png} & 
%\includegraphics[width=0.08\linewidth]{rebuttal/images/cid_000000314251_1.png} & 
%\includegraphics[width=0.08\linewidth]{rebuttal/images/boir_000000314251_0.png} & 
%\includegraphics[width=0.08\linewidth]{rebuttal/images/boir_000000314251_1.png} \\
(a) & (b) & (c) & (d) & (e) & (f) & (g) & (h) \\
\end{tabular}
\vspace*{-3mm}
}
%\caption{(a) Bbox Mask Loss framework: $\mathcal{L}_{pull}^{in}$ pulls instance center and soft-masked mean embeddings inside the box, $\mathcal{L}_{push}^{out}$ pushes pairwise instance-background embeddings, $\mathcal{L}_{push}^{inst}$ pushes pairwise instance embeddings. (b) Pipeline of instance keypoint head: backbone feature $f\in\mathbb{R}^{C,H,W}$ is sampled at center coordinates to retrieve instance-wise features $f^{p}\in\mathbb{R}^{C}$; Instance keypoint head (kpt) outputs instance-wise keypoint heatmap $k\in\mathbb{R}^{K,H,W}$. (c) Layer composition of instance keypoint head; \emph{LN} and \emph{IN}: Layer and instance normalization, respectively, $coord$: relative coordinates of the heatmap pixels; $f'\in\mathbb{R}^{C'\times H\times W}$: $f'\in\mathbb{R}^{C', H, W}$: a projection of $f$ by a single convolution layer. (d)-(g) Example predictions: (d) and (f) keypoint predictions of CID and BoIR, respectively. (e) and (g) feature map visualization of CID and BoIR, respectively.
%feature similarities from the instance centers of CID and BoIR, respectively.
%\vspace*{-4mm}
%}
\captionof{figure}{(a) Bbox Mask Loss framework: $\mathcal{L}_{pull}^{in}$ pulls instance center and soft-masked mean embeddings inside the box, $\mathcal{L}_{push}^{out}$ pushes pairwise instance-background embeddings, $\mathcal{L}_{push}^{inst}$ pushes pairwise instance embeddings. (b) Pipeline of instance keypoint head: backbone feature $f\in\mathbb{R}^{C,H,W}$ is sampled at center coordinates to retrieve instance-wise features $f^{p}\in\mathbb{R}^{C}$; Instance keypoint head (kpt) outputs instance-wise keypoint heatmap $k\in\mathbb{R}^{K,H,W}$. (c) Layer composition of instance keypoint head; \emph{LN} and \emph{IN}: Layer and instance normalization, respectively, $coord$: relative coordinates of the heatmap pixels; %$f'\in\mathbb{R}^{C'\times H\times W}$: 
$f'\in\mathbb{R}^{C', H, W}$: a projection of $f$ by a convolution layer. 
(d)-(h) Visualization of feature similarities from the center features of bounding boxes in (d): (e) and (f) CID feature similarities from A and B centers, respectively, (g) and (h) BoIR feature similarities.
%(d)-(g) Example predictions: (d) and (f) keypoint predictions of CID and BoIR, respectively. (e) and (g) feature map visualization of CID and BoIR, respectively.
%feature similarities from the instance centers of CID and BoIR, respectively.
\vspace*{-2mm}
}
\label{fig:fig_merged}
%\end{figure}
\end{strip}
%\end{figure*}


==> rebuttal/fig_mergedBackup.tex <==
%\begin{figure*}
%\begin{figure*}
\begin{strip}
%\begin{figure}[!ht]
\centering
\small{
\begin{tabular}{c@{}c@{}c c@{}c@{}c@{}c}
\includegraphics[width=0.132\linewidth]{rebuttal/pdfs/bml_framework.pdf} &
%\includegraphics[width=0.132\linewidth]{rebuttal/images/graphical_bml.png} &
\includegraphics[width=0.19\linewidth]{rebuttal/pdfs/pipeline.pdf}
 & %%%%%%%%%%%%%%%%%%%%
\includegraphics[width=0.28\linewidth]{rebuttal/pdfs/comp.pdf} &
\includegraphics[width=0.092\linewidth]{rebuttal/images/cid_116397_3.jpg} & 
\includegraphics[width=0.092\linewidth]{rebuttal/images/cid_116397_2.jpg} & 
\includegraphics[width=0.092\linewidth]{rebuttal/images/boir_116397_3.jpg} & 
\includegraphics[width=0.092\linewidth]{rebuttal/images/boir_116397_2.jpg} \\
%\includegraphics[width=0.10\linewidth]{rebuttal/images/graphical_bml.png} &
%\includegraphics[width=0.21\linewidth]{rebuttal/pdfs/pipeline.pdf}
% & %%%%%%%%%%%%%%%%%%%%
%\includegraphics[width=0.16\linewidth]{rebuttal/pdfs/comp.pdf}
%&
%\includegraphics[width=0.08\linewidth]{rebuttal/images/cid_000000314251_0.png} & 
%\includegraphics[width=0.08\linewidth]{rebuttal/images/cid_000000314251_1.png} & 
%\includegraphics[width=0.08\linewidth]{rebuttal/images/boir_000000314251_0.png} & 
%\includegraphics[width=0.08\linewidth]{rebuttal/images/boir_000000314251_1.png} \\
(a) & (b) & (c) & (d) & (e) & (f) & (g) \\
\end{tabular}
\vspace*{-3mm}
}
%\caption{(a) Bbox Mask Loss framework: $\mathcal{L}_{pull}^{in}$ pulls instance center and soft-masked mean embeddings inside the box, $\mathcal{L}_{push}^{out}$ pushes pairwise instance-background embeddings, $\mathcal{L}_{push}^{inst}$ pushes pairwise instance embeddings. (b) Pipeline of instance keypoint head: backbone feature $f\in\mathbb{R}^{C,H,W}$ is sampled at center coordinates to retrieve instance-wise features $f^{p}\in\mathbb{R}^{C}$; Instance keypoint head (kpt) outputs instance-wise keypoint heatmap $k\in\mathbb{R}^{K,H,W}$. (c) Layer composition of instance keypoint head; \emph{LN} and \emph{IN}: Layer and instance normalization, respectively, $coord$: relative coordinates of the heatmap pixels; $f'\in\mathbb{R}^{C'\times H\times W}$: $f'\in\mathbb{R}^{C', H, W}$: a projection of $f$ by a single convolution layer. (d)-(g) Example predictions: (d) and (f) keypoint predictions of CID and BoIR, respectively. (e) and (g) feature map visualization of CID and BoIR, respectively.
%feature similarities from the instance centers of CID and BoIR, respectively.
%\vspace*{-4mm}
%}
\captionof{figure}{(a) Bbox Mask Loss framework: $\mathcal{L}_{pull}^{in}$ pulls instance center and soft-masked mean embeddings inside the box, $\mathcal{L}_{push}^{out}$ pushes pairwise instance-background embeddings, $\mathcal{L}_{push}^{inst}$ pushes pairwise instance embeddings. (b) Pipeline of instance keypoint head: backbone feature $f\in\mathbb{R}^{C,H,W}$ is sampled at center coordinates to retrieve instance-wise features $f^{p}\in\mathbb{R}^{C}$; Instance keypoint head (kpt) outputs instance-wise keypoint heatmap $k\in\mathbb{R}^{K,H,W}$. (c) Layer composition of instance keypoint head; \emph{LN} and \emph{IN}: Layer and instance normalization, respectively, $coord$: relative coordinates of the heatmap pixels; %$f'\in\mathbb{R}^{C'\times H\times W}$: 
$f'\in\mathbb{R}^{C', H, W}$: a projection of $f$ by a single convolution layer. 
(d)-(g) Example predictions: (d) and (f) boxes from keypoint prediction of CID and BoIR, respectively. (e) and (g) t-SNE of CID and BoIR, respectively.
%(d)-(g) Example predictions: (d) and (f) keypoint predictions of CID and BoIR, respectively. (e) and (g) feature map visualization of CID and BoIR, respectively.
%feature similarities from the instance centers of CID and BoIR, respectively.
\vspace*{-4mm}
}
\label{fig:fig_merged}
%\end{figure}
\end{strip}
%\end{figure*}


==> rebuttal/framework_figure.tex <==
\begin{figure}
\centering
\includegraphics[width=0.24\linewidth]{rebuttal/images/graphical_bml.png}
\caption{Bbox Mask Loss framework.}
\label{fig:bml_framework}
\end{figure}

==> rebuttal/inst_kpt_head_comp.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\tikzstyle{connection}=[ultra thick,every node/.style={sloped,allow upside down, minimum size=1em},draw=\edgecolor,opacity=0.7]
% f
\node[canvas is xy plane at z=0] (fp) at (0,0,0) {$f^p$};

% c_att_linear
\node[shift={(1.0,1,0)},fill=green!40,minimum width=1,minimum height=1.4em,font=\small] at (fp.east) (c_linear) {Linear};
\node[shift={(0,-0.2,0)},minimum width=1,minimum height=1.4em,font=\small] at (c_linear.south) (c_linear_dim) {$C \rightarrow C'$};

% c_att_ln
\node[shift={(0.5,0,0)},fill=cyan!40,minimum width=1,minimum height=1.4em,font=\small] at (c_linear.east) (c_ln) {LN};

% c hadamard
\node[shift={(0.9,0,0)},minimum width=1,minimum height=1.4em,font=\small] at (c_ln) (c_hadamard) {$\otimes$};


% f^p
\node[shift={(2.935,0,0)},minimum width=1,minimum height=1.4em,font=\small] at (fp.east) (f) {$f'$};


% s linear
\node[shift={(1.0,-1.0,0)},fill=green!40,minimum width=1,minimum height=1.4em,font=\small] at (fp.east) (s_linear) {Linear};
\node[shift={(0,-0.2,0)},minimum width=1,minimum height=1.4em,font=\small] at (s_linear.south) (s_linear_dim) {$C \rightarrow C'$};

% s ln
\node[shift={(0.5,0,0)},fill=cyan!40,minimum width=1,minimum height=1.4em,font=\small] at (s_linear.east) (s_ln) {LN};

% s hadamard
\node[shift={(0.9,0,0)},minimum width=1,minimum height=1.4em,font=\small] at (s_ln) (s_hadamard) {$\otimes$};

% relative coords
\node[shift={(0,-0.5,0)},minimum width=1,minimum height=1.4em,font=\small] at (s_hadamard.south) (coord) {$coord$};

% s conv
\node[shift={(0.75,0,0)},fill=green!40,minimum width=1,minimum height=1.4em,font=\small] at (s_hadamard.east) (s_conv) {Conv};
\node[shift={(0,-0.2,0)},minimum width=1,minimum height=1.4em,font=\small] at (s_conv.south) (s_conv_dim) {$3 \rightarrow 1$};

% s in
\node[shift={(0.5,0,0)},fill=cyan!40,minimum width=1,minimum height=1.4em,font=\small] at (s_conv.east) (s_in) {IN};

% s hadamard 2
\node[shift={(0,1.0,0)},minimum width=1,minimum height=1.4em,font=\small] at (s_in) (s_hadamard2) {$\otimes$};

% fusion conv
\node[shift={(1.7,0,0)},fill=green!40,minimum width=1,minimum height=1.4em,font=\small] at (c_hadamard.east) (fusion_conv) {Conv};
\node[shift={(0,0.2,0)},minimum width=1,minimum height=1.4em,font=\small] at (fusion_conv.north) (fusion_conv_dim) {$2C' \rightarrow C'$};

% fusion in
\node[shift={(0.5,0,0)},fill=cyan!40,minimum width=1,minimum height=1.4em,font=\small] at (fusion_conv.east) (fusion_in) {IN};

% last layer
\node[shift={(0.7,0,0)},fill=green!40,minimum width=1,minimum height=1.4em,font=\small] at (fusion_in.east) (last_conv) {Conv};
\node[shift={(0,-0.2,0)},minimum width=1,minimum height=1.4em,font=\small] at (last_conv.south) (last_conv_dim) {$C' \rightarrow K$};

% connections
\draw [-Stealth]  (fp.east) -- (c_linear.west);
\draw [-Stealth]  (c_linear.east) -- (c_ln.west);
\draw [-Stealth]  (c_ln.east) -- (c_hadamard.west);
\draw [-Stealth]  (f.north) -- (c_hadamard.south);

\draw [-Stealth]  (fp.east) -- (s_linear.west);
\draw [-Stealth]  (s_linear.east) -- (s_ln.west);
\draw [-Stealth]  (s_ln.east) -- (s_hadamard.west);
\draw [-Stealth]  (f.south) -- (s_hadamard.north);
\draw [-Stealth]  (s_hadamard.east) -- (s_conv.west);
\draw [-Stealth]  (coord.east) -- (s_conv.west);
\draw [-Stealth]  (s_conv.east) -- (s_in.west);
\draw [-Stealth]  (s_in.north) -- (s_hadamard2.south);
\draw [-Stealth]  (f.east) -- (s_hadamard2.west);

\draw [-Stealth]  (c_hadamard.east) -- (fusion_conv.west);
\draw [-Stealth]  (s_hadamard2.north) -- (fusion_conv.south);

\draw [-Stealth]  (fusion_conv.east) -- (fusion_in.west);
\draw [-Stealth]  (fusion_in.east) -- (last_conv.west);

\end{tikzpicture}
\caption{Layer composition of instance keypoint head. 'Linear': linear layer, 'Conv': convolution layer, 'LN': Layer Normalization, 'IN': Instance Normalization, '$\otimes$': Hadamard product. '$coord$' refers to relative coordinates of the heatmap pixel indices. $f'\in\mathbb{R}^{C'\times H\times W}$ is a projection of $f$ by single convolution layer.}
\label{fig:inst_kpt_head_comp}
\end{figure}
